Let the Heads Talk: Beyond Diagonal Graph Attention

Sheaf Neural Networks generalize scalar-weighted message passing by replacing scalar edge weights with linear transport maps between local feature spaces. Yet the role of this matrix-valued transport is entangled with the broader sheaf-diffusion construction. We isolate the transport primitive through quiver representations and establish a direct connection with multi-head attention. Treating attention heads as coordinates of a local transport space reveals that standard multi-head attention implements diagonal edge maps: along each directed interaction, a source head can contribute only to the corresponding receiver head. Allowing off-diagonal entries instead enables edge-conditioned communication across heads before neighborhood aggregation. We show that this operation cannot, in general, be absorbed into a single shared linear map applied after aggregation. Building on this characterization, we introduce Topological Attention (Top-A), a multi-head attention that learns edge-dependent off-diagonal routes while preserving the original same-head paths and exactly recovering vanilla attention when the additional routing vanishes. We evaluate Top-A on relational reasoning, heterogeneous graph learning, and algorithmic reasoning, including out-of-distribution generalization, with heterophilic node classification as a contrast setting. The results show that cross-head transport is most useful when the task benefits from interaction-dependent transformations, while heterophily alone provides no systematic advantage. These findings identify edge-conditioned cross-head communication as a distinct computational primitive of matrix-valued transport.

==> chapters/version_31-08-2026/00_abstract.tex <==
% Previous abstract (retained for comparison):
% \begin{abstract}
% Graph neural networks have benefited from attention mechanisms and from extensions grounded in cellular sheaf theory. Graph attention assigns edge-dependent scalar weights to neighboring messages, while Sheaf Neural Networks use restriction maps between local vector spaces to induce matrix-valued edge couplings. We show that normalized multi-head graph attention is exactly realized by cellular-sheaf message passing: after embedding the head coordinates into a stalk space, restriction-induced coupling followed by a fixed readout reproduces the diagonal attention action before the usual output projection. This correspondence makes attention heads the observable coordinates of the stalk signal and identifies the off-diagonal head-space couplings absent from ordinary attention. It motivates \offdiag{}, a graph-attention mechanism that keeps the conventional attention coefficients on the diagonal and learns edge-conditioned off-diagonal terms that route messages between heads before neighborhood aggregation. The resulting perspective gives both a precise sheaf-theoretic account of multi-head graph attention and a practical design principle for cross-head communication.
% \end{abstract}

\begin{abstract}
\textcolor{red}{DISCLAIMER: le sezioni al momento "corrette" ma non necessariamente pulite o esposte bene sono dalla Section 1 to Section 5 e le Appendici che vedete al momento compilate. So bene che la prosa e i contenuti non sono ancora espressi in un formato da ICLR o submission, ma non sono molto bravo in quello, quindi liberi di modificare o rendere piu' bella e leggibile qualsiasi parte. Ho lasciato anche qualche commento qui e la'. Punti importanti al momento sono 1) non abbiamo un vero e proprio Related Works ma un Position in section 2.4, 2) forse necessitiamo di una spiegazione piu' approfondita della differenza tra una sheaf e copresehaf (magari in appendice), 3) le parti sulle sheaves (quelle dove mostriamo che e' fattorizzabile come restriction map) sono essenzialmente superflue le ho aggiunte cosi' siamo tutti contenti, ma non credo ci sara' spazio per tutto alla fine}
\end{abstract}


==> chapters/version_31-08-2026/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

The success of a graph neural network (GNN) often depends as much on how information is allowed to move across an edge as on how that information is represented at a node.  Graph attention networks make this choice adaptive: each receiver learns how strongly to weight the messages arriving from its neighbors \citep{velickovic2018graph,brody2022attentive}. Multi-head attention enriches this mechanism by learning several such weighting patterns in parallel and has become a standard component of graph transformers and message-passing architectures \citep{yun2019graph, gilmer2017neural}. Yet the edgewise action of standard multi-head attention remains highly structured. Different heads may attend to different neighbors, but a value produced by one head remains within that head while crossing an edge. Cross-head interaction through the usual output projection occurs only after the incoming messages have already been aggregated.

Sheaf Neural Networks (SNNs) approach graph communication from a different direction. Rather than describing an interaction only through a scalar weight, they equip local feature spaces with linear maps that can transform information as it moves between neighboring nodes \citep{hansen2020toward,bodnar2022neural}. This matrix-valued view of transport provides additional freedom in how local representations interact and was motivated in part by the challenges posed by heterophilic graphs \citep{bodnar2022neural,barbero2022sheaf}. It has since motivated a broader family of neural sheaf architectures with increasingly expressive local
transport mechanisms \citep{barbero2022sheafconnection, borgi2025polynomial, bamberger2025bundle, ribeiro2026cooperative}. Recent empirical evidence, however, suggests that the source of these gains should be identified more carefully. On classical heterophilic benchmarks, Identity Sheaf Networks, in which restriction maps are fixed to the identity,
can perform comparably to several learned SNN variants, questioning whether learned non-trivial restriction maps are themselves responsible for the
reported improvements \citep{caralt2026necessity}. On newer heterophilic benchmarks from  \cite{platonov2023critical}, including \textsc{roman-empire} and \textsc{amazon-ratings},
strong attention and graph-transformer baselines can likewise match or outperform classical neural sheaf diffusion variants. These observations suggest a more focused question than whether sheaf-based models are
universally advantageous: \emph{which forms of local transport provide a useful inductive bias, and which of them are absent from standard
message-passing architectures?}

We investigate this question through multi-head attention. The head decomposition already provides a natural coordinate system for examining how
information is transported along an edge: each head propagates its own value representation independently, so the corresponding edge transport is diagonal across heads. What is absent from this standard edge operator is a mechanism for information carried by one source head to enter another head while the message is still associated with a particular edge. This observation connects attention naturally to the local-transport perspective developed in sheaf and copresheaf neural networks \citep{hajij2026copresheaf}. We use this connection not to replace attention with a general sheaf diffusion, but to isolate a specific architectural choice: \emph{whether different head subspaces should be allowed to communicate on individual edges before neighborhood aggregation}. This leads to \textsc{TopA} (Topological Attention), a minimal extension of multi-head attention that retains the original same-head attention paths while introducing edge-conditioned routing between heads. Cross-head interaction has also been explored in Transformer attention by mixing or dynamically composing attention scores and weights
\citep{shazeer2020talking,xiao2024improving}. Our focus is complementary: \textsc{TopA} acts directly on the value-head representation carried by each
directed graph edge, before contributions from different neighbors are aggregated, preserving the identity of the incoming interaction when cross-head routing is applied.

Our aim is therefore to test a specific transport bias rather than a broad claim about the superiority of matrix-valued message passing. We first use a controlled feature-partition setting in which complementary information is
separated across heads, allowing the role of cross-head communication to be examined directly. We then evaluate the same mechanism on the CLRS
algorithmic reasoning benchmark \citep{velickovic2022clrs}, where a shared graph processor must propagate and combine intermediate information across a diverse collection of algorithms. Together, these settings allow us to study
both whether the proposed routing performs its intended communication role and when that inductive bias is useful in more demanding reasoning tasks.

Our \textbf{contributions} are: \textcolor{red}{(to polish)}
\begin{enumerate}[leftmargin=1.5em]

\item We identify normalized multi-head graph attention, prior to its output
projection, as diagonal transport on the native head space. We formalize this
view through directed graph copresheaves and corresponding
restriction-induced cellular-sheaf realizations, placing attention within a
broader family of matrix-valued local transport operators.

\item Guided by this characterization, we introduce \textsc{TopA}, an
edge-conditioned residual extension that preserves the current attention
coefficients on the diagonal while enabling cross-head routing before
neighborhood aggregation.

\item We characterize when edge-specific pre-aggregation routing can be
represented by shared post-aggregation mixing, and evaluate the resulting
inductive bias through controlled headwise feature separation and across the
CLRS algorithmic-reasoning benchmark.

\end{enumerate}

% ---- figure ----
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{img/OffDiag_VisualAbstract.pdf}
\caption{\emph{Topological Attention (TOPA) Overview}. Standard multi-head graph attention transports information independently within each head, with each head propagating its own value representation independently across an edge. TOPA preserves these original attention paths while introducing edge-conditioned cross-head routing, allowing information from one source head to contribute to a different receiver head before neighborhood aggregation. Because routing depends on each directed edge, different interactions can induce distinct patterns of head communication. After the edgewise messages are aggregated over the neighborhood, the usual shared output projection mixes the resulting head representations.
}
\label{fig:offdiag-visual-abstract}
\end{figure}


==> chapters/version_31-08-2026/01_introduction_v2.tex <==
\section{Introduction}
\label{sec:introduction}

Sheaf Neural Networks (SNNs) provide a view of graph learning in which communication is governed not only by which neighbors interact, but also by how information is transformed along each interaction \citep{hansen2020toward,bodnar2022neural}. Rather than relying exclusively on scalar edge weights, SNNs use restriction maps to induce matrix-valued transformations between local representation spaces, an idea that has motivated a growing family of neural sheaf architectures \citep{barbero2022sheaf, barbero2022sheafconnection, borgi2025polynomial,bamberger2025bundle,ribeiro2026cooperative}. At the level of message-passing transport, however, this construction can be viewed as a structured specialization of a more general object: a representation of the graph quiver\todo{forse spiegherei brevemente cosa e'}, or equivalently a vector-space-valued graph copresheaf, where directed edges carry source-to-target linear maps \citep{hajij2026copresheaf}. Cellular sheaves realize such transport through restriction-map factorizations and intermediate edge stalks. While much of the neural-sheaf literature exploits the resulting matrix-valued transport, the additional constraints imposed by this specifically sheaf-theoretic factorization are rarely used as an architectural principle in their own right. This motivates taking quiver representations as the broader starting point, with SNNs forming a structured subfamily and other graph architectures arising through different constraints on the same local transport space.

Viewed through this lens, multi-head graph attention is another, particularly constrained specialization. Attention adaptively determines how strongly a receiver weights its neighbors, with multiple heads learning different interaction patterns \citep{velickovic2018graph,brody2022attentive}, but along each edge every head transports its value independently. Cross-head interaction through the usual output projection occurs only after messages from different neighbors have been aggregated and is shared across all such interactions. General quiver transport can instead couple local coordinates while each edge contribution is still distinguishable. Identifying these coordinates with attention heads turns this additional freedom into \emph{edge-specific cross-head communication}: information from one source head may contribute to a different receiver head before neighborhood aggregation. Such transport admits a cellular-sheaf realization but does not require the additional sheaf structure. This perspective is complementary to Talking-Heads and related approaches, which mix attention scores or weights across heads \citep{shazeer2020talking,xiao2024improving}; here, communication acts directly on the values transported by each graph edge.

Motivated by this observation, we introduce \textsc{TopA} \todo{Top-A?} (\emph{Topological Attention}), an edge-conditioned extension of multi-head graph attention that changes \emph{where} and \emph{how} cross-head communication occurs. \textsc{TopA} preserves the original same-head attention paths while allowing head routing to depend on each directed interaction before neighborhood aggregation. Different neighbors of the same receiver may therefore induce different patterns of head communication, unlike the shared post-aggregation mixing of standard multi-head attention. Our construction neither replaces attention with an SNN nor requires the structural constraints of cellular sheaves; instead, the quiver perspective exposes \emph{edge-specific, pre-aggregation cross-head transport} as an additional degree of freedom of multi-head attention. We evaluate this inductive bias through controlled feature partitioning, where complementary information is deliberately separated across heads, and on the CLRS algorithmic reasoning benchmark \citep{velickovic2022clrs}, where graph processors must propagate and combine intermediate information across diverse algorithmic tasks.

Our \textbf{contributions} are:
\begin{enumerate}[leftmargin=1.5em]

\item We reinterpret the matrix-valued local transport underlying Sheaf Neural Networks through graph-quiver representations, viewing the sheaf construction as a structured, restriction-induced realization of the more general source-to-target transport available in a graph copresheaf.

\item Within this broader framework, we characterize multi-head graph attention as a constrained specialization in which heads are transported independently along each edge, exposing edge-specific, pre-aggregation cross-head transport as an additional degree of freedom.

\item Guided by this characterization, we introduce \textsc{TopA}, an edge-conditioned extension of multi-head attention that preserves the original same-head attention paths while enabling interaction-dependent communication between heads before neighborhood aggregation, without requiring cellular-sheaf constraints.

\item We characterize when edge-specific pre-aggregation routing can be reproduced by shared post-aggregation mixing, and evaluate the resulting inductive bias through controlled headwise feature partitioning and the CLRS algorithmic-reasoning benchmark.

\end{enumerate}



% \section{Introduction}
% \label{sec:introduction}

% Many graph neural architectures can be viewed as different ways of specifying how information is transported along the interactions of a graph. A particularly general language for describing such local transport is provided by representations of graph quivers, where nodes carry local representation spaces and directed edges specify how information is transformed from a sender to a receiver \citep{hajij2026copresheaf}. From this perspective, familiar graph-learning mechanisms need not be regarded as fundamentally separate constructions. Instead, they can be interpreted as imposing different structural constraints on a common family of edgewise transport operators.

% Multi-head graph attention provides an important example. Attention learns how strongly each receiver should weight the information arriving from its neighbors, with different heads producing different interaction patterns \citep{velickovic2018graph,brody2022attentive}. Yet, despite this adaptivity, the local action of standard multi-head attention is highly constrained. Each head transports its own value representation independently: information produced within one head remains associated with that same head while traversing an edge. In the language of quiver representations, ordinary multi-head attention therefore corresponds to a restricted form of local transport in which the different head coordinates do not interact during message propagation. Cross-head communication, when present through the usual output projection, occurs only after messages from the different neighbors have already been aggregated.

% This characterization suggests a natural connection with cellular sheaves. Sheaf-based graph models also describe local information exchange through linear maps associated with graph incidences, but allow substantially richer transformations between local representation spaces \citep{hansen2020toward,bodnar2022neural}. Viewed through the underlying quiver representation, the distinction is one of structure rather than principle: standard attention occupies a constrained subfamily of local transport, whereas sheaf-induced transport can realize more general matrix-valued interactions. When the local coordinates are identified with attention heads, these additional degrees of freedom acquire a particularly simple interpretation: information carried by one source head can be transferred into a different receiver head while the message is still associated with an individual edge.

% This gives a new perspective on \emph{head communication}. Multi-head architectures are typically designed so that heads process information in parallel and are combined only at later stages. Previous works such as Talking-Heads attention have shown that interactions between heads can be beneficial by mixing attention scores or weights \citep{shazeer2020talking,xiao2024improving}. The quiver and sheaf viewpoints expose a complementary possibility: heads can communicate directly at the level of the values transported by each graph edge. Rather than asking only how much a receiver should attend to a neighbor, the model can also determine how the information associated with that particular interaction should move between head subspaces before neighborhood aggregation.

% This perspective motivates \textsc{TopA} (\emph{Topological Attention}), an extension of multi-head graph attention that introduces edge-conditioned communication between heads while retaining the original attention mechanism. Conceptually, \textsc{TopA} starts from the constrained transport already implemented by ordinary attention and selectively relaxes the restriction that keeps different heads independent along an edge. The standard same-head attention paths are preserved, while additional routes allow information from one source head to contribute to another receiver head. Because these routes are conditioned on the directed interaction being processed, different edges may induce different patterns of head communication.

% The distinction between this mechanism and conventional head mixing is important. A shared output projection can combine head representations only after all incoming messages have been summarized at a node. At that stage, the model no longer has access to each neighbor contribution as an independent interaction. \textsc{TopA}, instead, performs head communication before this aggregation takes place. It can therefore transform the contribution of one sender differently from that of another sender, even when both messages arrive at the same receiver. The additional expressivity is thus not merely the ability to mix heads, but the ability to perform \emph{edge-specific head talking} while individual interactions are still distinguishable.

% Our construction can consequently be understood through a simple hierarchy. Quiver representations provide the general language of directed local transport. Under the structural constraints realized by ordinary multi-head attention, this transport reduces to independent same-head communication. Cellular-sheaf constructions provide a richer realization in which local coordinates may interact, revealing cross-head communication as a natural additional degree of freedom. \textsc{TopA} isolates precisely this degree of freedom and incorporates it into existing attention architectures without replacing their original attention computation.

% Our aim is not to argue that general matrix-valued transport should universally replace standard attention. Rather, we ask whether this particular relaxation of the attention operator provides a useful inductive bias when information must be combined across head subspaces. We investigate this question in two complementary settings. First, we introduce a controlled feature-partitioning experiment in which complementary information is deliberately separated across heads, making the role of cross-head communication directly observable. Second, we evaluate the same mechanism on the CLRS algorithmic reasoning benchmark \citep{velickovic2022clrs}, where graph processors must propagate and combine intermediate information across a diverse collection of algorithms. These experiments allow us to study both whether \textsc{TopA} performs its intended communication role and when such edge-specific head interaction is beneficial in more challenging reasoning tasks.

% Our \textbf{contributions} are:
% \begin{enumerate}[leftmargin=1.5em]

% \item We develop a unified view of multi-head graph communication through representations of graph quivers, showing that ordinary normalized multi-head attention corresponds to a structurally constrained form of local transport in which head coordinates propagate independently along each edge.

% \item We connect this characterization to cellular-sheaf transport, showing how relaxing the corresponding structural constraints exposes cross-head communication as a natural additional degree of freedom in the local transport space.

% \item Guided by this connection, we introduce \textsc{TopA}, an edge-conditioned extension of multi-head attention that preserves the original same-head attention paths while enabling information to be routed between different heads before neighborhood aggregation.

% \item We characterize the distinction between edge-specific pre-aggregation routing and conventional shared post-aggregation head mixing, and evaluate the resulting inductive bias through controlled headwise feature partitioning and the CLRS algorithmic-reasoning benchmark.

% \end{enumerate}

% ---- figure ----
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{img/OffDiag_VisualAbstract.pdf}
\caption{\emph{Topological Attention (TOPA) Overview}. From the perspective of graph-quiver representations, standard multi-head attention implements a constrained form of local transport in which each head propagates independently along an edge. TOPA preserves these original same-head attention paths while introducing edge-conditioned communication between different heads before neighborhood aggregation. Different directed interactions may therefore induce different patterns of head communication. Once the edgewise messages have been aggregated, computation returns to the standard attention backbone and its shared output projection.}
\label{fig:offdiag-visual-abstract}
\end{figure}

==> chapters/version_31-08-2026/02_background_positioning.tex <==
\section{Background and Positioning}
\label{sec:background}

\todo[inline]{\textbf{(i)} non spieghiamo mai le SNN. \textbf{(ii)} In generale, sembra che in questa sezione introduciamo gia' un po' di intuizioni/concetti nuovi, mentre qui secondo me dovrebbe esserci solo il background che ti permette di capire il resto del paper. (pero' potrei aver letto velocemente)}

\paragraph{Graph Attention as Message Passing.}
\label{sec:background-attention}
Graph attention weights the messages arriving at each node according to their
relevance to the receiver. By using the convention \(i\leftarrow j\) for a
message along the directed edge \(e=(j\to i)\), for head \(h\), let
\(s_{i\leftarrow j}^{(h)}\) denote the unnormalized attention score.
Normalization over the incoming neighborhood of \(i\) then gives:
\begin{equation}
    \alpha_{i\leftarrow j}^{(h)}
    =
    \frac{
        \exp s_{i\leftarrow j}^{(h)}
    }{
        \sum_{k\in\mathcal{N}(i)}
        \exp s_{i\leftarrow k}^{(h)}
    }
    \label{eq:attention-normalization}
\end{equation}
The scores may arise from query--key interactions or learned functions of the
endpoint representations
\citep{velickovic2018graph,brody2022attentive,shi2021masked}. Our analysis
begins after score construction and normalization and is therefore agnostic
to this choice. Let each of the \(H\) heads have width \(C\), and collect the projected
values at node \(j\) as \(V_j\in\R^{H\times C}\), with row
\(V_j^{(h)}\) corresponding to head \(h\). The attention coefficients
associated with the same edge define the diagonal head-space operator:
\begin{equation}
    D_{i\leftarrow j}
    =
    \operatorname{Diag}
    \left(
        \alpha_{i\leftarrow j}^{(1)},\ldots,
        \alpha_{i\leftarrow j}^{(H)}
    \right)
    \in\R^{H\times H}
    \label{eq:diagonal-attention}
\end{equation}
The pre-readout multi-head update can then be written as:
\begin{equation}
    M_i^{\att}
    =
    \sum_{j\in\mathcal{N}(i)}
    D_{i\leftarrow j}V_j
    \label{eq:mha}
\end{equation}
This notation separates the head and within-head axes. Under
\(\R^{H\times C}\simeq\R^H\otimes\R^C\), the corresponding edge action is
\(D_{i\leftarrow j}\otimes I_C\): the attention operator acts on the
\(H\)-dimensional head space while applying each head coefficient uniformly
across its \(C\) value coordinates. Our construction will modify this
head-space transport while leaving the within-head coordinates unchanged.
The usual output projection \(W_O\), when present, acts only after the
incoming edge messages have been aggregated.


\paragraph{Directed Local Transport as a Graph Copresheaf.}
\label{sec:background-copresheaf}
Equation~\ref{eq:mha} is a special case of directed message passing in
which each edge carries a linear map between local feature spaces. A natural
language for this structure is a representation of the graph quiver, or
equivalently a vector-space-valued graph copresheaf
\citep{hajij2026copresheaf}.

Let \(G=(\mathcal{V},\mathcal{E},s,t)\) be a directed graph \todo{ where $\mathcal{V}$ is ..., $\mathcal{E}$ represents ....}. A graph
copresheaf \(\mathcal{Q}\) assigns a vector space \(\mathcal{Q}(i)\) to each
vertex and a linear map:
\begin{equation}
    T_e:
    \mathcal{Q}(s(e))
    \longrightarrow
    \mathcal{Q}(t(e))
    \label{eq:copresheaf-arrow}
\end{equation}
to each directed edge \(e\).\footnote{
Equivalently, a representation of the graph quiver extends to a functor from
the path category of \(G\) to \(\mathbf{Vect}_{\mathbb{R}}\), with maps along
directed paths obtained by composition. Appendix~\ref{app:quiver-path-category}
gives the full construction and clarifies that opposite arrows need not be
inverses.
}
When the local spaces have dimension \(d\), the corresponding incoming
transport is:
\begin{equation}
    M_i^{\mathcal{Q}}
    =
    \sum_{e:t(e)=i}
    T_e X_{s(e)},
    \qquad
    X_{s(e)}\in\R^{d\times C}
    \label{eq:copresheaf-message-passing}
\end{equation}\todo{darei anche una intuizione a parole di cosa e' una copresheaf oltre alla formula}
Opposite computational directions correspond to different edge maps. Thus,
when both \(j\to i\) and \(i\to j\) are present,
\(T_{j\to i}\) and \(T_{i\to j}\) need not be related, matching the
directional structure of attention. In neural message passing, these maps may depend on the current hidden state. At layer \(\ell\), we may therefore write
\(T_e^{(\ell)}=T_e^{(\ell)}(X^{(\ell)})\). For every fixed network state,
the resulting collection of maps defines a graph copresheaf; we refer to
this state-dependent construction as a \emph{dynamic graph copresheaf}.
Attention is one such example: its edge maps depend on the current
representations and, through neighborhood normalization, on the incoming
neighborhood of the receiver. Appendix~\ref{app:dynamic-copresheaf}
formalizes this state-dependent interpretation.


\paragraph{Restriction-induced Cellular-Sheaf Transport.}
\label{sec:background-sheaf}
The copresheaf description specifies source-to-target transport directly. Cellular sheaves provide a complementary factorized representation in which the same transport is mediated through an intermediate edge space. A cellular sheaf \(\mathcal{F}\) assigns vector spaces, or \emph{stalks}, to
vertices and edges together with linear restriction maps for their incidences
\citep{hansen2020toward,bodnar2022neural}. To represent directed computation,
we associate each directed interaction with its own \(1\)-cell. Thus, if both
\(j\to i\) and \(i\to j\) occur, they are represented by distinct edge
cells and may use independent restriction maps. Consider a directed edge \(e=(j\to i)\). Let \(\mathcal{F}(j)\) and
\(\mathcal{F}(i)\) denote the sender and receiver vertex stalks, respectively,
and let \(\mathcal{F}(e)\) be the corresponding edge stalk. We write:
\begin{equation}
    S_e:
    \mathcal{F}(j)\longrightarrow\mathcal{F}(e),
    \qquad
    R_e:
    \mathcal{F}(i)\longrightarrow\mathcal{F}(e)
    \label{eq:source-target-restrictions}
\end{equation}
for the sender and receiver restriction maps. With the Euclidean inner
products used throughout, they induce the source-to-target transport:
\begin{equation}
    T_e
    =
    R_e^\top S_e:
    \mathcal{F}(j)\longrightarrow\mathcal{F}(i)
    \label{eq:sheaf-induced-transport}
\end{equation}
so that the edge message takes the form:
\begin{equation}
    m_e
    =
    R_e^\top S_e X_j
    \label{eq:sheaf-edge-message}
\end{equation}
The edge stalk therefore provides an intermediate space through which the
sender representation is mapped before being transferred into the receiver
stalk. Using distinct edge cells for the two computational directions allows the
induced transports to vary independently. If instead a single undirected
edge and the same pair of restriction maps are used in both directions, the
reverse transport is the transpose of the forward one; the explicit
derivation is given in
Appendix~\ref{app:directed-sheaf-reciprocity}. For later use, let \(B_s\) and \(B_t\) collect the sender and receiver
restriction maps across all directed edges. Their cross-incidence composition
acts as:
\begin{equation}
    \left(
        B_t^\ast B_s X
    \right)_i
    =
    \sum_{e:t(e)=i}
    R_e^\top S_e X_{s(e)}
    \label{eq:directed-cross-incidence}
\end{equation}
Appendix~\ref{app:global-incidence} gives the corresponding construction on
the direct sums of vertex and edge stalks. The operator \(B_t^\ast B_s\) is the directed source-to-target component of the degree-zero sheaf Laplacian; its precise relation to \(L_{\mathcal F}=\delta^\ast\delta\) is given in
Appendix~\ref{app:sheaf-laplacian-relation}. Here we use this cross term
directly as a generally non-self-adjoint transport operator; our analysis
does not rely on sheaf-diffusion dynamics or spectral properties. Finally, a factorization \(T_e=R_e^\top S_e\) is generally non-unique. In
the constructions below, we choose restriction maps that make the
computational decomposition of the corresponding edge operator explicit.


\paragraph{Positioning and Related Architectures.}
\label{sec:background-positioning}
Copresheaf Topological Neural Networks provide a general framework in which
directed interactions carry linear maps between local vector spaces
\citep{hajij2026copresheaf}. We use this copresheaf, or quiver, perspective
as the primary description of the edge operators considered here.
Cellular sheaves provide a complementary realization of these operators
through restriction maps and intermediate edge stalks. Our contribution is therefore not the introduction of matrix-valued edge maps themselves, but their specialization to the coordinate structure already present in multi-head attention. In particular, the next section shows that
ordinary attention occupies the diagonal part of this head-space transport,
which exposes cross-head transport as a specific missing degree of freedom. 
Related architectures also introduce interactions across heads or
edge-conditioned feature transformations. Talking-Heads attention and dynamic
head-composition methods mix attention scores or weights across heads
\citep{shazeer2020talking,xiao2024improving}, while edge-conditioned graph
convolutions generate feature-space filters from individual interactions
\citep{simonovsky2017dynamic}. \textsc{TopA} instead acts on the value-head
representation carried by each directed edge before neighborhood aggregation,
while retaining the original diagonal attention operator as the same-head
transport. \todo{volendo possiamo rimandare ad una sezione in appendice dove aggiungiamo una sezione di related work classica per far contenti i revisori}


==> chapters/version_31-08-2026/03_exact_representation.tex <==
\section{Attention as Diagonal Head-Space Transport}
\label{sec:representation}

The \(H\) parallel heads of multi-head attention naturally define an
\(H\)-dimensional local space. We therefore set:
\begin{equation}
    \mathcal{Q}(i)=\R^H
    \label{eq:head-local-space}
\end{equation}
at every node and treat the \(C\) coordinates within each head as parallel
signals. The full value representation is thus
\(\R^H\otimes\R^C\)\todo{otimes = ?}, with edge transport acting on the head factor. In this
native basis, coordinate \(h\) corresponds directly to attention head \(h\).


\subsection{Ordinary attention is diagonal on head space}
\label{sec:attention-diagonal}
\todo[inline]{non partirei a bomba dal teorema. Metterei un preambolo per rendere tutto piu' fluido}
\begin{proposition}[Multi-Head Attention as Diagonal Head-space Transport]
\label{prop:attention-diagonal-transport}
Consider a normalized \(H\)-head graph-attention layer with
\(V_j\in\R^{H\times C}\). For each directed edge \(e=(j\to i)\), define:
\begin{equation}
    T_e^{\att}
    =
    D_e
    =
    \operatorname{Diag}
    \left(
        \alpha_e^{(1)},\ldots,\alpha_e^{(H)}
    \right)
    \label{eq:attention-arrow-map}
\end{equation}
Then:
\begin{equation}
    \sum_{e:t(e)=i}
    T_e^{\att}V_{s(e)}
    =
    M_i^{\att}
    \label{eq:attention-copresheaf-update}
\end{equation}
Hence, prior to any post-aggregation readout, normalized multi-head attention
is exactly a diagonal directed transport on its native head space.
\end{proposition}

The proposition follows directly from Equation~\ref{eq:mha}; a complete
componentwise proof is given in
Appendix~\ref{app:proof-attention-diagonal}. Its consequence is immediate at
the level of individual heads:
\begin{equation}
    \left[D_eV_j\right]^{(r)}
    =
    \alpha_e^{(r)}V_j^{(r)}
    \label{eq:attention-diagonal-action}
\end{equation}
A value carried by source head \(r\) therefore contributes only to the
corresponding receiver-head coordinate. Different heads may assign different
weights to the same neighbor, but the edge operator itself does not transfer
values between head subspaces. The usual output projection \(W_O\), when present, may subsequently mix the aggregated heads. Its position in the computation is important: \(D_e\) acts
on each incoming edge separately, whereas \(W_O\) is applied only after those
edge contributions have been combined. Moreover, for each receiver and head,
the diagonal entries of the incoming \(D_e\) are non-negative and sum to one
by attention normalization. This diagonal characterization is tied to the head decomposition explicitly realized by the architecture. It is preserved under arbitrary relabelings of
the heads, while an unrestricted change of basis in \(\R^H\) need not preserve
diagonality (see Appendix~\ref{app:head-basis}).


\subsection{Restriction-induced realization of attention}
\label{sec:attention-restriction-realization}

The same diagonal operator admits an exact cellular-sheaf realization. Since
the entries of \(D_e\) are non-negative, its principal square root
\(D_e^{1/2}\) is well defined.

\begin{proposition}[Restriction-induced Realization of Attention]
\label{prop:attention-restriction-realization}
For a directed edge \(e=(j\to i)\), let: 
\[
    \mathcal{F}(i)
    =
    \mathcal{F}(j)
    =
    \mathcal{F}(e)
    =
    \R^H
\]
and choose: 
\begin{equation}
    S_e
    =
    R_e
    =
    D_e^{1/2}
    \label{eq:attention-restrictions}
\end{equation}
Then:
\begin{equation}
    R_e^\top S_e
    =
    D_e
    \label{eq:attention-restriction-factorization}
\end{equation}
and the resulting directed cross-incidence transport reproduces the
multi-head attention update exactly.
\end{proposition}
Indeed:
\begin{equation}
        R_e^\top S_e
    =
    \left(D_e^{1/2}\right)^\top D_e^{1/2}
    =
    D_e
\end{equation}
The restriction maps therefore provide a factorization of the attention
operator after its coefficients have been computed; they are not additional
learned parameters of the attention layer. The square-root construction is
one convenient symmetric realization among many possible factorizations. Because \(D_e\) depends on the current hidden representations, the
corresponding realization is instantiated dynamically at each layer and
forward pass. A complete proof, including the induced global
cross-incidence update, is given in
Appendix~\ref{app:proof-attention-sheaf}.


\subsection{From diagonal to matrix-valued transport}
\label{sec:matrix-transport}

The head-space view makes the missing interaction explicit. A general
directed transport \(T_e\in\R^{H\times H}\) acts as:
\begin{equation}
    \left[T_eV_j\right]^{(r)}
    =
    \sum_{s=1}^{H}
    T_e^{rs}V_j^{(s)} 
    \label{eq:matrix-valued-head-transport}
\end{equation}
Diagonal entries describe same-head communication, while an off-diagonal
entry \(T_e^{rs}\), with \(r\neq s\), routes information from source head
\(s\) into receiver head \(r\) on that edge. We consider this generalization only along the head factor. On the full value space, the corresponding action remains:
\begin{equation}
    T_e\otimes I_C
    \label{eq:head-space-only-transport}
\end{equation}
rather than an arbitrary transformation in \(\R^{HC\times HC}\). This
isolates cross-head communication without simultaneously introducing
edge-dependent mixing across the \(C\) within-head channels. Standard attention therefore uses only diagonal head-space transport, with non-negative coefficients normalized across the incoming edges of each receiver. Section~\ref{sec:native} extends this operator by adding edge-conditioned off-diagonal terms, while keeping the original diagonal attention paths unchanged.



==> chapters/version_31-08-2026/04_native_width_routing.tex <==
\section{\textsc{TopA}: Edge-Conditioned Routing Between Heads}
\label{sec:native}

Section~\ref{sec:representation} shows that standard multi-head attention
acts diagonally on its native head space. \textsc{TopA} relaxes this constraint
in the smallest structured way needed to introduce cross-head communication:
it retains the diagonal attention operator and adds edge-conditioned routes
between different heads before neighborhood aggregation.


\subsection{Residual head-space transport}
\label{sec:offdiag-operator}

For each directed edge \(e=(j\to i)\), let
\(\Omega_e\in\R^{H\times H}\) be a routing matrix satisfying $\operatorname{diag}(\Omega_e)=0$.
We define the \textsc{TopA} edge operator as:
\begin{equation}
    T_e
    =
    D_e
    \left(
        I_H+\lambda\Omega_e
    \right),
    \qquad
    \lambda\geq0
    \label{eq:offdiag-transport}
\end{equation}
where \(\lambda\) controls the strength of the residual routing path. The
receiver update is:
\begin{equation}
    M_i^{\offdiag}
    =
    \sum_{e:t(e)=i}
    D_e
    \left(
        I_H+\lambda\Omega_e
    \right)
    V_{s(e)}
    \label{eq:offdiag-aggregation}
\end{equation}
For receiver head \(r\):
\begin{equation}
    \left[M_i^{\offdiag}\right]^{(r)}
    =
    \sum_{j\in\mathcal{N}(i)}
    \alpha_{i\leftarrow j}^{(r)}
    \left[
        V_j^{(r)}
        +
        \lambda
        \sum_{\substack{s=1\\s\neq r}}^{H}
        \Omega_{i\leftarrow j}^{rs}V_j^{(s)}
    \right]
    \label{eq:offdiag-components}
\end{equation}
The first term is the standard same-head message, while
\(\Omega_{i\leftarrow j}^{rs}\) routes information from source head \(s\)
into receiver head \(r\) on the particular edge \(j\to i\). The ordering in Equation~\ref{eq:offdiag-transport} is deliberate. Because \(D_e\) acts from the left,
\(\alpha_{i\leftarrow j}^{(r)}\) gates the complete message entering
receiver head \(r\), including contributions routed from other source heads.
Thus the original attention coefficient retains its receiver-side
interpretation, while \(\Omega_e\) determines how source-head values are
combined within that gate. Placing \(D_e\) on the right would instead gate
each routed contribution by its source-head coefficient. The equivalent
componentwise implementation is given in
Appendix~\ref{app:implementation-order}.

\subsection{Structural properties}
\label{sec:offdiag-preservation}
The residual parameterization preserves the attention paths already present
in the backbone and confines the additional edgewise capacity to cross-head
transport.
\begin{proposition}[Structural Properties of \textsc{TopA}]
\label{prop:offdiag-structural}
\label{prop:diagonal-preservation}
\label{prop:vanilla-recovery}
Let:
\begin{equation}
     T_e
    =
    D_e
    \left(
        I_H+\lambda\Omega_e
    \right),
    \qquad
    \operatorname{diag}(\Omega_e)=0
\end{equation}
Then:
\begin{equation}
    \operatorname{diag}(T_e)
    =
    \operatorname{diag}(D_e)
    \label{eq:diagonal-preservation}
\end{equation}
and, if \(\Omega_e=0\), we have:
\begin{equation}
    T_e=D_e
    \label{eq:vanilla-recovery}
\end{equation}
Hence \textsc{TopA} preserves the current same-head attention coefficients and
recovers standard attention exactly when the routing branch vanishes.
\end{proposition}
These properties follow immediately from:
\begin{equation}
    T_e
    =
    D_e+\lambda D_e\Omega_e
\end{equation}
since \(D_e\) is diagonal and \(\Omega_e\) has zero diagonal. A complete
proof, including the layer-local interpretation of diagonal preservation, is
given in Appendix~\ref{app:proof-offdiag-structural}.
The operator family is also closed under permutations of the head labels,
and standard attention forms its zero-routing subfamily; see
Appendices~\ref{app:offdiag-head-permutation}
and~\ref{app:nested-operator-families}.


\subsection{Learning edge-conditioned routes}
\label{sec:offdiag-parameterization}

A shared head-mixing matrix would permit communication between heads but
would apply the same transformation to every interaction. \textsc{TopA} instead
generates the routing matrix from the directed edge currently being
processed. Let \(\xi_e\in\R^p\) denote an edge descriptor constructed from the current
processor state. A learned map:
\begin{equation}
    g_\theta:
    \R^p
    \longrightarrow
    \R^{H\times H}
\end{equation}
maps this descriptor to a head-space matrix, from which we define:
\begin{equation}
    \Omega_e
    =
    \operatorname{off}
    \left(
        \tanh g_\theta(\xi_e)
    \right)
    \label{eq:offdiag-generator}
\end{equation}
with:
\[
    \operatorname{off}(A)
    =
    A-\operatorname{Diag}(\operatorname{diag}(A))
\]
The off-diagonal projection prevents the routing branch from modifying the
diagonal attention paths, while the elementwise \(\tanh\) bounds the route
values and permits both positive and negative contributions. This
parameterization also yields a simple worst-case bound on
\(\|T_e-D_e\|_2\), derived in
Appendix~\ref{app:offdiag-residual-bound}. Because \(\xi_e\) describes a directed interaction, opposite computational directions may produce different routing matrices. Their corresponding
cellular-sheaf realizations are therefore instantiated independently; see
Appendix~\ref{app:offdiag-sheaf-directionality}. For each fixed network state, the operators:
\begin{equation}
    T_e
    =
    D_e
    \left(
        I_H+\lambda\Omega_e
    \right)
    :
    \R^H\longrightarrow\R^H
\end{equation}
form the edge maps of the dynamic graph copresheaf introduced in
Section~\ref{sec:background-copresheaf}. The associated cellular-sheaf
realization inherits the same state dependence
(Appendix~\ref{app:offdiag-sheaf-state-dependence}). In the implementation, the routing projection is initialized at zero, so training begins from the corresponding vanilla attention computation.
Section~\ref{sec:offdiag-initialization-baseline} gives the concrete
initialization and baseline-equivalence details.


\subsection{Cellular-sheaf realization of \textsc{TopA}}
\label{sec:offdiag-sheaf-realization}
The operator \(T_e\) is used directly during message passing. It also admits
a cellular-sheaf realization that makes the standard and residual paths
explicit. 
For each directed edge \(e\), consider the edge stalk:
\begin{equation}
    \mathcal{F}(e)
    =
    \R^H_{\mathrm{att}}
    \oplus
    \R^H_{\mathrm{route}}
    \cong
    \R^{2H}
    \label{eq:offdiag-edge-stalk}
\end{equation}
with vertex stalks \(\mathcal{F}(i)\cong\R^H\). Choose:
\begin{equation}
    R_e
    =
    \begin{bmatrix}
        D_e^{1/2}\\[1mm]
        \sqrt{\lambda}\,D_e
    \end{bmatrix},
    \qquad
    S_e
    =
    \begin{bmatrix}
        D_e^{1/2}\\[1mm]
        \sqrt{\lambda}\,\Omega_e
    \end{bmatrix}
    \label{eq:offdiag-restrictions}
\end{equation}
The dimensional construction of these maps is detailed in Appendix~\ref{app:offdiag-direct-sum}.
\begin{proposition}[Restriction-induced Realization of \textsc{TopA}]
\label{prop:offdiag-sheaf-realization}
The restriction maps in Equation~\eqref{eq:offdiag-restrictions} satisfy:
\begin{equation}
    R_e^\top S_e
    =
    D_e
    \left(
        I_H+\lambda\Omega_e
    \right)
    =
    T_e
    \label{eq:offdiag-factorization}
\end{equation}
Hence the complete \textsc{TopA} aggregation is exactly realized by the
directed cross-incidence transport \(B_t^\ast B_s\).
\end{proposition}
The direct-sum construction mirrors the residual architecture. Its first
component induces the standard contribution
\(D_eV_{s(e)}\), while the second induces the routed term
\(\lambda D_e\Omega_eV_{s(e)}\). The full derivation, global
cross-incidence form, and lift to \(T_e\otimes I_C\) are given in
Appendices~\ref{app:proof-offdiag-sheaf},
\ref{app:offdiag-path-decomposition}, and
\ref{app:offdiag-full-value-space}. This factorization is a realization of the implemented operator rather than a separate learned parameterization. The backbone produces \(D_e\), the
routing branch produces \(\Omega_e\), and the restriction maps above are
constructed algebraically from these quantities
(Appendix~\ref{app:offdiag-induced-not-learned}).
The realization is not unique. The \(2H\)-dimensional direct sum is chosen
because it exposes the standard and residual paths separately, not because
it is minimal or canonical
(Appendix~\ref{app:offdiag-factorization-nonunique}). When the routing path
vanishes, the construction reduces to the attention realization of
Section~\ref{sec:attention-restriction-realization}; see
Appendix~\ref{app:offdiag-sheaf-vanilla-limit}.


\subsection{Why routing before aggregation is different}
\label{sec:offdiag-postmix}
A shared post-aggregation map, such as the usual output projection \(W_O\)
when present, acts only after the incoming edge contributions have been
combined. \textsc{TopA} instead applies an edge-specific head-space
transformation while each sender contribution is still available separately. We now characterize exactly when these two operations can coincide. Let
\(v_j=\operatorname{hvec}(V_j)\in\R^{HC}\) denote the head-major
vectorization of the sender values, and define:
\begin{equation}
    \overline{D}_{i\leftarrow j}
    =
    D_{i\leftarrow j}\otimes I_C,
    \qquad
    \overline{T}_{i\leftarrow j}
    =
    T_{i\leftarrow j}\otimes I_C
    \label{eq:lifted-edge-operators}
\end{equation}
The corresponding vectorization identity is given in
Appendix~\ref{app:postmix-lifting}. 
\begin{theorem}[Shared Post-aggregation Equivalence]
\label{thm:postmix-non-equivalence}
Fix a receiver \(i\). There exists a single linear map
\(A\in\R^{HC\times HC}\) such that:
\begin{equation}
    \sum_{j\in\mathcal{N}(i)}
    \overline{T}_{i\leftarrow j}v_j
    =
    A
    \sum_{j\in\mathcal{N}(i)}
    \overline{D}_{i\leftarrow j}v_j
    \label{eq:postmix-equivalence}
\end{equation}
for every collection
\(\{v_j\}_{j\in\mathcal{N}(i)}\) if and only if:
\begin{equation}
    \overline{T}_{i\leftarrow j}
    =
    A\,
    \overline{D}_{i\leftarrow j}
    \qquad
    \text{for every }j\in\mathcal{N}(i)
    \label{eq:common-left-factor}
\end{equation}
\end{theorem}

The condition follows by considering one sender at a time: equality for all
possible sender values requires the same left factor \(A\) to reproduce every
incoming edge operator individually. The full necessity-and-sufficiency proof
is given in Appendix~\ref{app:proof-postmix}. For \textsc{TopA}, if the incoming attention coefficients are strictly positive,
as for unmasked edges with finite softmax logits, each
\(D_{i\leftarrow j}\) is invertible. The required post-aggregation map must
then satisfy:
\begin{equation}
    A
    =
    \left[
        D_{i\leftarrow j}
        \left(
            I_H+\lambda\Omega_{i\leftarrow j}
        \right)
        D_{i\leftarrow j}^{-1}
    \right]
    \otimes I_C
    \label{eq:offdiag-common-factor}
\end{equation}
for every incoming edge. A single post-aggregation map therefore exists only
when these induced transformations agree across all senders, a constraint
not imposed by edge-conditioned routing. Appendix~\ref{app:postmix-offdiag}
gives the full derivation and covers non-invertible attention operators as
well. The distinction is therefore one of computational access: post-aggregation
mixing acts on a neighborhood summary, whereas \textsc{TopA} can transform
each sender contribution separately before the sum. A minimal two-edge
counterexample is given in
Appendix~\ref{app:postmix-counterexample}, and the precise scope of the
operator-level result is discussed in
Appendix~\ref{app:postmix-scope}. Section~\ref{sec:methodology} next describes how this operator is instantiated in GATv2 and graph Transformer backbones.




==> chapters/version_31-08-2026/05_architectural_istantiation.tex <==
\section{Architectural Instantiation}
\label{sec:methodology}

Section~\ref{sec:native} defines \textsc{TopA} independently of the attention
mechanism used to construct \(D_e\). We now instantiate the same operator in
GATv2 and a graph Transformer. In both cases, the backbone retains its
original attention scores, normalization, value projections, and
post-aggregation update; \textsc{TopA} modifies only the edge-level value
transport before neighborhood aggregation.


\subsection{General integration}
\label{sec:architecture-general}

For each directed edge \(e=(j\to i)\), the backbone provides the normalized
attention operator \(D_e\), sender values \(V_j\in\R^{H\times C}\), and a
directed descriptor \(\xi_e\in\R^p\) constructed from representations
already available to the attention layer. In the implementations considered here, the map
\(g_\theta\) from Section~\ref{sec:offdiag-parameterization} is a dense linear
projection:
\begin{equation}
    G_e
    =
    \operatorname{reshape}_{H\times H}
    \left(
        W_\Omega\xi_e+b_\Omega
    \right),
    \qquad
    \Omega_e
    =
    \operatorname{off}
    \left(
        \tanh G_e
    \right)
    \label{eq:architecture-routing}
\end{equation}
The resulting operator $T_e
    =
    D_e
    \left(
        I_H+\lambda\Omega_e
    \right)$, is applied to \(V_j\) before the usual neighborhood aggregation. Computation
then returns to the original backbone, leaving its residual connections,
nonlinearities, normalization, and subsequent processor updates unchanged. The two instantiations below therefore differ only in the construction of \(D_e\), \(V_j\), and the routing descriptor \(\xi_e\). Unless stated otherwise, we use \(\lambda=1\).

\subsection{\textsc{TopA}-GATv2}
\label{sec:offdiag-gatv2}

Our first instantiation augments the GATv2 processor
\citep{brody2022attentive}. Let \(z_i\) denote the representation entering
the processor layer. For the directed interaction \(i\leftarrow j\), our
GATv2 backbone forms the pre-attention context:
\begin{equation}
    u_{i\leftarrow j}
    =
    W_{\mathrm{recv}}z_i
    +
    W_{\mathrm{send}}z_j
    +
    W_E e_{i\leftarrow j}
    +
    W_G g
    \label{eq:gatv2-edge-context}
\end{equation}
where the edge and graph terms are omitted when unavailable. This context is
used by the backbone to construct its standard headwise attention scores and
the corresponding receiver-normalized operator
\(D_{i\leftarrow j}\). The routing branch reuses the same directed interaction and defines:
\begin{equation}
    \xi_{i\leftarrow j}
    =
    \sigma_{\mathrm{LReLU}}
    \left(
        u_{i\leftarrow j}
    \right)
    \label{eq:gatv2-routing-descriptor}
\end{equation}
Equation~\ref{eq:architecture-routing} then maps the full descriptor to
\(\Omega_{i\leftarrow j}\). The sender values are transported by:
\begin{equation}
    D_{i\leftarrow j}
    \left(
        I_H+\lambda\Omega_{i\leftarrow j}
    \right)
    V_j
\end{equation}
before being summed over the incoming neighborhood. The remainder of the GATv2 processor is unchanged: the aggregated heads are returned to the original concatenation, residual, activation, and
normalization path. Thus the only additional operation is the
edge-conditioned cross-head transport inserted between value construction
and neighborhood aggregation.


\subsection{\textsc{TopA} Graph Transformer}
\label{sec:offdiag-gt}

Our second instantiation applies the same transport rule to a graph
Transformer backbone \citep{shi2021masked}. The backbone constructs the usual
headwise queries, keys, and values. For a directed interaction
\(i\leftarrow j\), available edge and graph representations are incorporated
into the sender key:
\begin{equation}
    K_{i\leftarrow j}
    =
    K_j
    +
    E_{i\leftarrow j}
    +
    G
    \label{eq:gt-conditioned-key}
\end{equation}
Standard scaled dot-product attention between
\(Q_i\) and \(K_{i\leftarrow j}\), followed by receiver-wise normalization,
defines \(D_{i\leftarrow j}\). For the routing branch, we retain the full directed query--key context and define:
\begin{equation}
    \xi_{i\leftarrow j}
    =
    \operatorname{vec}
    \left(
        Q_i
        \,\Vert\,
        K_{i\leftarrow j}
    \right)
    \label{eq:gt-routing-descriptor}
\end{equation}
where \(\Vert\) denotes concatenation along the feature axis. This descriptor
is projected through Equation~\ref{eq:architecture-routing} to obtain
\(\Omega_{i\leftarrow j}\), which acts on the sender values through the same
receiver-gated transport used in \textsc{TopA}-GATv2. After neighborhood aggregation, computation returns to the original Transformer readout, residual path, nonlinearities, and normalization. The
two backbone instantiations therefore differ in their attention mechanisms
and routing descriptors while implementing the same edge-level operator
\(D_e(I_H+\lambda\Omega_e)\).


\subsection{Initialization and baseline equivalence}
\label{sec:offdiag-initialization-baseline}
The residual parameterization provides an exact vanilla reference point. In
the baseline configuration, the routing branch is disabled and $T_e=D_e$, so the model contains no routing parameters and otherwise retains the same backbone architecture. For the active \textsc{TopA} model, we initialize:
\begin{equation}
    W_\Omega=0,
    \qquad
    b_\Omega=0
    \label{eq:routing-zero-initialization}
\end{equation}
It follows that \(G_e=0\), \(\Omega_e=0\), and \(T_e=D_e\) for every edge.
With matched shared-backbone parameters, vanilla attention and \textsc{TopA}
therefore implement exactly the same function at initialization. The full
forward-equivalence argument is given in
Appendix~\ref{app:implementation-vanilla-reference}. Zero initialization does not prevent the routing branch from learning: \(\tanh'(0)=1\), so for \(\lambda>0\) the off-diagonal routing parameters can
receive first-order gradients at the initial solution. Appendix~\ref{app:implementation-gradient}
gives the corresponding derivative calculation, including the fact that the
new routing path contributes no additional initial gradient to the
descriptor-producing backbone when \(W_\Omega=0\). We additionally verify parity between vanilla and zero-initialized \textsc{TopA} at the level of edge messages, aggregated representations, and
model outputs. The complete set of implementation checks is reported in
Appendix~\ref{app:implementation-parity}.


\subsection{Computational cost}
\label{sec:offdiag-complexity}

The additional cost arises from generating and applying one dense
\(H\times H\) routing matrix for each directed edge. For a descriptor of
width \(p\), the projection in Equation~\eqref{eq:architecture-routing}
contains \(pH^2\) weights and, when used, \(H^2\) biases. Exact allocated and
active parameter counts, together with the backbone-specific descriptor
dimensions, are given in Appendix~\ref{app:implementation-parameters}.
Generating the routing matrix costs \(O(pH^2)\) per edge, while applying
\(\Omega_e\in\R^{H\times H}\) to \(V_j\in\R^{H\times C}\) costs \(O(H^2C)\). Excluding computations already required to construct \(\xi_e\), the additional graph-level cost is therefore:
\begin{equation}
    O\!\left(
        |\mathcal{E}|\,pH^2
        +
        |\mathcal{E}|\,H^2C
    \right)
    \label{eq:offdiag-complexity}
\end{equation}
with \(O(|\mathcal{E}|H^2)\) additional memory when all routing matrices are
materialized. A more detailed operation and memory accounting is provided in
Appendix~\ref{app:implementation-complexity}. The quadratic dependence on \(H\) reflects the dense set of possible routes between source and receiver heads. Since the architectures studied here use
a small number of heads, we retain the dense parameterization rather than
imposing an additional sparsity or low-rank structure. Appendix~\ref{app:implementation-correspondence} summarizes the complete correspondence between the implemented routing pipeline and the operator analyzed in Sections~\ref{sec:native} and~\ref{sec:methodology}.



==> chapters/version_31-08-2026/06_experimental_design.tex <==
\section{Experimental Evaluation}
\label{sec:design}

Having established attention as the diagonal case and isolated non-diagonal head-space routing as the added operation, we test whether these edge-level routes matter when information is separated across heads and across algorithmic tasks. The experiments address two complementary questions.

\paragraph{RQ1: Sensitivity to Feature Partitioning.}
Standard multi-head attention lets every head construct its representation from the full node feature vector, although the heads aggregate edge messages independently. We introduce a controlled condition in which each head receives a disjoint subset of the input features. Comparing \gatv{} and a graph Transformer with their \textsc{TopA} variants tests whether edge-level cross-head routes reduce sensitivity to this enforced separation. We use Roman Empire, Amazon Ratings, Squirrel Filtered, and Chameleon Filtered from the heterophily benchmark of \citet{platonov2023critical}.

\paragraph{RQ2: Task-dependent Utility on CLRS.}
We compare \gatv{} and \gats{} on the CLRS algorithmic-reasoning benchmark \citep{velickovic2022clrs}. This study asks whether off-diagonal routing is useful across a broad collection of algorithms and, equally importantly, where it does not help.

The feature-partition study uses the same fixed data splits and equal hyperparameter-search budgets for every model and condition. The CLRS study uses paired random seeds, official task-specific metrics, and the same checkpoint-selection rule for both processors. We report node-classification accuracy and CLRS scores as percentages, with differences in percentage points. Full architectures, search spaces, optimization settings, and aggregation procedures appear in Appendix~\ref{app:protocols}. Code and experiment scripts will be released with the paper.


==> chapters/version_31-08-2026/07_clrs.tex <==
\section{Evaluation on the CLRS Benchmark}
\label{sec:clrs}
\input{tables/clrs_macros.tex}

CLRS is an established benchmark for learning to execute classical algorithms \citep{velickovic2022clrs}. Its tasks cover graph algorithms, sorting, searching, dynamic programming, geometry, string matching, and scheduling, with task-specific official metrics. We train a separate processor for each task and compare \gatv{} with \gats{} using the canonical data splits, identical hidden width, paired random seeds, and best-validation checkpoint selection. Ten paired seeds are available for 29 tasks. \texttt{optimal\_bst} is omitted because both variants encounter the same implementation failure before evaluation. Appendix~\ref{app:protocols} gives the full training configuration. The CLRS variant uses direct OffDiag (Equation~\ref{eq:direct-offdiag}): it augments the standard diagonal attention operator with a learned, directed off-diagonal residual before neighborhood aggregation. This is a routing relaxation rather than the factored node-classification parameterization.

\noindent\textbf{Aggregate Performance.}
Averaging first over seeds and then over the 29 completed tasks, the official CLRS score increases from \(49.17\%\) for \gatv{} to \(55.04\%\) for \gats{}, a mean improvement of \(5.87\) percentage points. A hierarchical task-and-seed bootstrap gives \([\ClrsBootLo,\ClrsBootHi]\) points. The median task-level improvement is \(1.04\) points. Across the 290 paired runs, \gats{} scores higher in 175, equally in 20, and lower in 95. Mean performance improves on 21 tasks, decreases on seven, and is unchanged at displayed precision on BFS.

\input{tables/clrs_families.tex}

\noindent\textbf{Task Heterogeneity. }
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{\input{img/tikz/clrs_forest.tex}}
\caption{Task-level difference in official CLRS score. Points show mean paired differences over ten seeds; bars show 95\% \(t\)-intervals of the paired differences. Positive values favor \gats{}, and the gray \texttt{optimal\_bst} row marks a shared implementation failure.}
\label{fig:clrs-forest}
\end{figure}
The gains are strongly heterogeneous. Binary search improves by \(46.03\) points, insertion sort by \(43.56\), Prim by \(21.57\), quicksort by \(21.12\), and Graham scan by \(17.88\). In contrast, heapsort changes by \(-4.68\) points, Kruskal by \(-4.08\), and strongly connected components by \(-3.33\). The Prim--Kruskal and quicksort--heapsort contrasts show that routing is not uniformly helpful even within related algorithm families. Appendix~\ref{app:clrs} reports all task means, standard deviations, paired intervals, and seed-level direction counts.


==> chapters/version_31-08-2026/08_feature_splitting.tex <==
\section{Controlled Feature Partitioning}
\label{sec:feature}
Each head in standard graph attention constructs and aggregates its edge messages independently. Although the output projection can combine the resulting head summaries, it acts only after neighborhood aggregation and cannot exchange information between heads on a particular edge. Feature partitioning makes this separation explicit and tests whether \textsc{TopA}'s pre-aggregation routes compensate for it.

\noindent\textbf{Construction.}
In the \emph{dense} condition, every head constructs its query, key, and value representations---or the corresponding GATv2 endpoint and value representations---from the complete node feature vector. In the \emph{partitioned} condition, the features are divided into \(H\) disjoint subsets and head \(h\) constructs those representations only from subset \(h\). The standard attention computation is otherwise retained at every layer. Vanilla heads remain independent until the final readout; \textsc{TopA} can transfer an edge message from source head \(s\) to receiver head \(r\) before messages from different neighbors are aggregated. We evaluate both conditions on four datasets with ten fixed splits. Every model--condition pair receives the same 36-point architecture-search budget, and test accuracy is measured at the best-validation checkpoint. Appendix~\ref{app:protocols} specifies the search and selection procedure. Let \(O_{\rm part}\) and \(O_{\rm dense}\) denote the \textsc{TopA} accuracies and \(V_{\rm part}\), \(V_{\rm dense}\) those of the vanilla backbone. We report the interaction:
\begin{equation}
  \featureDelta=
  (O_{\rm part}-O_{\rm dense})
  -(V_{\rm part}-V_{\rm dense})
  \label{eq:interaction}
\end{equation}
Positive values indicate that \textsc{TopA} is less sensitive to feature partitioning than its backbone.

\input{tables/feature_main.tex}

\noindent\textbf{Results.}
Roman Empire provides the clearest evidence for the proposed communication role. Partitioning reduces \gatv{} accuracy by \(9.6\) percentage points, whereas \gats{} changes by only \(-0.2\) points, yielding \(\featureDelta=+9.4\) points. The corresponding graph-Transformer interaction is \(+2.7\) points. The interaction is positive in seven of eight dataset--backbone comparisons; the remaining Chameleon/\gt{} comparison is \(-0.4\) points. The effects on Amazon Ratings, Squirrel Filtered, and Chameleon Filtered are smaller relative to the observed split-to-split variation, making Roman Empire the strongest controlled result. The matched-grid analysis in Appendix~\ref{app:fixed-feature-partition} shows the same broad ordering without relying only on the selected configurations.
\todoresult{Add paired confidence intervals for \(\featureDelta\) from the per-split results and repeat the analysis with random feature-to-head partitions.}


==> chapters/version_31-08-2026/09_discussion_conclusion.tex <==
\section{Discussion}
\label{sec:discussion}

The central theoretical point is an inclusion rather than an analogy. At the normalized message-operator level, and up to fixed lift and readout maps on the stalk coordinates, multi-head graph attention is recovered through restriction-induced sheaf message passing with a diagonal induced action on the observable head coordinates. A general matrix-valued edge action can additionally couple these coordinates. \textsc{TopA} turns precisely this extra degree of freedom into a graph-attention mechanism: a message produced by one head may enter another head before neighborhood aggregation. Because the transformation varies across edges and precedes the output readout, it cannot generally be reduced to \(W_O\). The cellular-sheaf connection and the practical mechanism play different roles. Theorem~\ref{thm:attention-sheaf} is an exact representation of normalized attention through restriction-induced coupling. The node-classification implementation uses a related endpoint factorization, while the CLRS implementation predicts a general directed off-diagonal residual. Both empirical models instantiate the same diagonal-plus-off-diagonal operator. The experiments therefore do not show that reciprocal sheaf structure causes the observed gains. 
The feature-partition experiment tests the intended communication capability: \textsc{TopA} is less sensitive when each head receives only part of the node features, most clearly on Roman Empire. CLRS tests the same routing mechanism across algorithmic tasks. Performance improves substantially on some search, sorting, graph, and geometry tasks but declines on others. Cross-head routing is therefore a selective inductive bias rather than a uniformly beneficial addition. Our scope is limited to graph-supported attention with equal head widths. The representation theorem operates on coefficients after neighborhood normalization and may define a data-dependent sheaf. Dense \textsc{TopA} routing costs \(O(|E|H^2C)\) to apply and introduces additional parameters; the CLRS comparison is width matched but not parameter matched. The feature partition follows the given feature order and retains a dense final decoder. These limitations restrict our empirical conclusions to the evaluated routing models and settings.

\section{Conclusion}
\label{sec:conclusion}
We showed that normalized multi-head graph attention is exactly realized through cellular-sheaf message passing with fixed lift and readout maps before the usual output projection. Attention heads index the observable stalk coordinates, and ordinary attention induces a diagonal action on them; matrix-valued transport supplies edge-conditioned communication between different coordinates. \textsc{TopA} turns this additional operation into a practical graph-attention mechanism by preserving normalized attention on the diagonal and adding cross-head routes before neighborhood aggregation. Controlled feature partitioning and CLRS show that this capability can matter, while the task-level variation clarifies that it is an inductive bias rather than a universal improvement. The correspondence therefore separates the diagonal operator already present in attention from the cross-head couplings available in sheaf message passing.


==> chapters/version_31-08-2026/10_routing_analysis.tex <==
\section{Analysis of Learned Head Routing}
\label{sec:analysis}

The predictive experiments establish when \textsc{TopA} helps, but the learned matrices can also reveal how the model uses cross-head routes. We focus on Roman Empire, where feature partitioning produces the largest interaction, and use Amazon Ratings as a secondary case. The analysis combines descriptive matrix statistics with test-time interventions.

\subsection{Off-diagonal utilization}

For each layer and edge, write \(P=D+O\) and measure the fraction of operator energy outside the diagonal:
\begin{equation}
  \rho_{\off}(P)=
  \frac{\|O\|_F^2}
       {\|D\|_F^2+\|O\|_F^2+\epsilon}
  \label{eq:offdiag-energy}
\end{equation}
We additionally summarize signed and absolute route magnitude, row entropy, the singular spectrum, and effective rank. Layer summaries average over edges within each evaluation split before aggregating across splits.

\todoresult{Insert layer-wise off-diagonal energy, route magnitude, entropy, and effective-rank results for dense and partitioned checkpoints.}

\subsection{Functional interventions}
We compare the intact operator with four test-time interventions: replacing \(P\) by \(D\) (removing off-diagonal routes), replacing it by the identity, shuffling \(O\) across edges within each graph, and replacing \(O\) by its layer mean. For each split, we report the intact-minus-intervened accuracy and a paired 95\% confidence interval. A larger diagonal-removal effect in the partitioned condition would connect the predictive interaction to the learned cross-head channel.
\todoresult{Insert paired intervention effects for Roman Empire and Amazon Ratings.}

\subsection{Organization of head representations}
At the value, routed-message, and aggregated-head stages, we flatten each head over a common node/edge sample axis and compute the full head covariance and correlation matrices, mean absolute off-diagonal correlation, and covariance effective rank. Linear CKA compares head activation matrices across dense and partitioned models after aligning heads on a held-out reference split. These statistics describe representation organization; they are not treated as causal evidence.

\todoresult{Insert covariance, correlation, and CKA analyses by layer for matched dense and partitioned \textsc{TopA} checkpoints.}

\subsection{Routing and predictive effects}
Finally, we relate partition robustness and CLRS task-level differences to off-diagonal energy and intervention sensitivity, reporting positive, neutral, and negative cases under the same selection rule.
\todoresult{Insert the association between routing statistics, feature-partition interactions, and CLRS task effects.}


==> img/tikz/clrs_forest.tex <==
\begin{tikzpicture}[x=0.071cm,y=0.235cm,font=\tiny]
\path[use as bounding box] (-62,-2.8) rectangle (68,30.2);
\draw[gray!60] (0,-1)--(0,29.5);
\draw[gray!35] (-40,-0.4)--(-40,29.1);
\node[anchor=north] at (-40,-0.7) {-40};
\draw[gray!35] (-20,-0.4)--(-20,29.1);
\node[anchor=north] at (-20,-0.7) {-20};
\draw[gray!35] (0,-0.4)--(0,29.1);
\node[anchor=north] at (0,-0.7) {+0};
\draw[gray!35] (20,-0.4)--(20,29.1);
\node[anchor=north] at (20,-0.7) {+20};
\draw[gray!35] (40,-0.4)--(40,29.1);
\node[anchor=north] at (40,-0.7) {+40};
\draw[gray!35] (60,-0.4)--(60,29.1);
\node[anchor=north] at (60,-0.7) {+60};
\node[anchor=east] at (-43,0) {Heapsort};
\draw[orange!80!black,line width=.45pt] (-31.4487,0)--(22.0834,0);
\draw[orange!80!black] (-31.4487,-0.16)--(-31.4487,0.16);
\draw[orange!80!black] (22.0834,-0.16)--(22.0834,0.16);
\fill[orange!80!black] (-4.6826,0) circle (0.55pt);
\node[anchor=east] at (-43,1) {Kruskal};
\draw[orange!80!black,line width=.45pt] (-8.9188,1)--(0.7593,1);
\draw[orange!80!black] (-8.9188,0.84)--(-8.9188,1.16);
\draw[orange!80!black] (0.7593,0.84)--(0.7593,1.16);
\fill[orange!80!black] (-4.0797,1) circle (0.55pt);
\node[anchor=east] at (-43,2) {SCC};
\draw[orange!80!black,line width=.45pt] (-10.1797,2)--(3.5098,2);
\draw[orange!80!black] (-10.1797,1.84)--(-10.1797,2.16);
\draw[orange!80!black] (3.5098,1.84)--(3.5098,2.16);
\fill[orange!80!black] (-3.3350,2) circle (0.55pt);
\node[anchor=east] at (-43,3) {Activity selector};
\draw[orange!80!black,line width=.45pt] (-13.3474,3)--(6.9564,3);
\draw[orange!80!black] (-13.3474,2.84)--(-13.3474,3.16);
\draw[orange!80!black] (6.9564,2.84)--(6.9564,3.16);
\fill[orange!80!black] (-3.1955,3) circle (0.55pt);
\node[anchor=east] at (-43,4) {Articulation points};
\draw[orange!80!black,line width=.45pt] (-15.3271,4)--(9.2874,4);
\draw[orange!80!black] (-15.3271,3.84)--(-15.3271,4.16);
\draw[orange!80!black] (9.2874,3.84)--(9.2874,4.16);
\fill[orange!80!black] (-3.0198,4) circle (0.55pt);
\node[anchor=east] at (-43,5) {Segments intersect};
\draw[orange!80!black,line width=.45pt] (-1.7445,5)--(0.3171,5);
\draw[orange!80!black] (-1.7445,4.84)--(-1.7445,5.16);
\draw[orange!80!black] (0.3171,4.84)--(0.3171,5.16);
\fill[orange!80!black] (-0.7137,5) circle (0.55pt);
\node[anchor=east] at (-43,6) {Task scheduling};
\draw[orange!80!black,line width=.45pt] (-2.6164,6)--(1.7938,6);
\draw[orange!80!black] (-2.6164,5.84)--(-2.6164,6.16);
\draw[orange!80!black] (1.7938,5.84)--(1.7938,6.16);
\fill[orange!80!black] (-0.4113,6) circle (0.55pt);
\node[anchor=east] at (-43,7) {BFS};
\draw[orange!80!black,line width=.45pt] (-0.0247,7)--(0.0149,7);
\draw[orange!80!black] (-0.0247,6.84)--(-0.0247,7.16);
\draw[orange!80!black] (0.0149,6.84)--(0.0149,7.16);
\fill[orange!80!black] (-0.0049,7) circle (0.55pt);
\node[anchor=east] at (-43,8) {Quickselect};
\draw[blue!70!black,line width=.45pt] (-0.0247,8)--(0.0637,8);
\draw[blue!70!black] (-0.0247,7.84)--(-0.0247,8.16);
\draw[blue!70!black] (0.0637,7.84)--(0.0637,8.16);
\fill[blue!70!black] (0.0195,8) circle (0.55pt);
\node[anchor=east] at (-43,9) {Jarvis march};
\draw[blue!70!black,line width=.45pt] (-2.9225,9)--(3.0591,9);
\draw[blue!70!black] (-2.9225,8.84)--(-2.9225,9.16);
\draw[blue!70!black] (3.0591,8.84)--(3.0591,9.16);
\fill[blue!70!black] (0.0683,9) circle (0.55pt);
\node[anchor=east] at (-43,10) {Naive string};
\draw[blue!70!black,line width=.45pt] (-1.4273,10)--(1.6715,10);
\draw[blue!70!black] (-1.4273,9.84)--(-1.4273,10.16);
\draw[blue!70!black] (1.6715,9.84)--(1.6715,10.16);
\fill[blue!70!black] (0.1221,10) circle (0.55pt);
\node[anchor=east] at (-43,11) {KMP};
\draw[blue!70!black,line width=.45pt] (-0.0325,11)--(0.5501,11);
\draw[blue!70!black] (-0.0325,10.84)--(-0.0325,11.16);
\draw[blue!70!black] (0.5501,10.84)--(0.5501,11.16);
\fill[blue!70!black] (0.2588,11) circle (0.55pt);
\node[anchor=east] at (-43,12) {LCS length};
\draw[blue!70!black,line width=.45pt] (-0.4978,12)--(1.0257,12);
\draw[blue!70!black] (-0.4978,11.84)--(-0.4978,12.16);
\draw[blue!70!black] (1.0257,11.84)--(1.0257,12.16);
\fill[blue!70!black] (0.2640,12) circle (0.55pt);
\node[anchor=east] at (-43,13) {Bridges};
\draw[blue!70!black,line width=.45pt] (-4.8929,13)--(6.7024,13);
\draw[blue!70!black] (-4.8929,12.84)--(-4.8929,13.16);
\draw[blue!70!black] (6.7024,12.84)--(6.7024,13.16);
\fill[blue!70!black] (0.9047,13) circle (0.55pt);
\node[anchor=east] at (-43,14) {Kadane};
\draw[blue!70!black,line width=.45pt] (-1.1778,14)--(3.2677,14);
\draw[blue!70!black] (-1.1778,13.84)--(-1.1778,14.16);
\draw[blue!70!black] (3.2677,13.84)--(3.2677,14.16);
\fill[blue!70!black] (1.0449,14) circle (0.55pt);
\node[anchor=east] at (-43,15) {Minimum};
\draw[blue!70!black,line width=.45pt] (-2.1308,15)--(6.7499,15);
\draw[blue!70!black] (-2.1308,14.84)--(-2.1308,15.16);
\draw[blue!70!black] (6.7499,14.84)--(6.7499,15.16);
\fill[blue!70!black] (2.3096,15) circle (0.55pt);
\node[anchor=east] at (-43,16) {DAG shortest paths};
\draw[blue!70!black,line width=.45pt] (0.6484,16)--(4.1172,16);
\draw[blue!70!black] (0.6484,15.84)--(0.6484,16.16);
\draw[blue!70!black] (4.1172,15.84)--(4.1172,16.16);
\fill[blue!70!black] (2.3828,16) circle (0.55pt);
\node[anchor=east] at (-43,17) {Bellman--Ford};
\draw[blue!70!black,line width=.45pt] (1.5520,17)--(3.9363,17);
\draw[blue!70!black] (1.5520,16.84)--(1.5520,17.16);
\draw[blue!70!black] (3.9363,16.84)--(3.9363,17.16);
\fill[blue!70!black] (2.7441,17) circle (0.55pt);
\node[anchor=east] at (-43,18) {Floyd--Warshall};
\draw[blue!70!black,line width=.45pt] (-6.1140,18)--(11.6633,18);
\draw[blue!70!black] (-6.1140,17.84)--(-6.1140,18.16);
\draw[blue!70!black] (11.6633,17.84)--(11.6633,18.16);
\fill[blue!70!black] (2.7747,18) circle (0.55pt);
\node[anchor=east] at (-43,19) {DFS};
\draw[blue!70!black,line width=.45pt] (-2.7422,19)--(9.4414,19);
\draw[blue!70!black] (-2.7422,18.84)--(-2.7422,19.16);
\draw[blue!70!black] (9.4414,18.84)--(9.4414,19.16);
\fill[blue!70!black] (3.3496,19) circle (0.55pt);
\node[anchor=east] at (-43,20) {Topological sort};
\draw[blue!70!black,line width=.45pt] (-9.6423,20)--(17.5817,20);
\draw[blue!70!black] (-9.6423,19.84)--(-9.6423,20.16);
\draw[blue!70!black] (17.5817,19.84)--(17.5817,20.16);
\fill[blue!70!black] (3.9697,20) circle (0.55pt);
\node[anchor=east] at (-43,21) {Matrix chain};
\draw[blue!70!black,line width=.45pt] (0.8594,21)--(9.4287,21);
\draw[blue!70!black] (0.8594,20.84)--(0.8594,21.16);
\draw[blue!70!black] (9.4287,20.84)--(9.4287,21.16);
\fill[blue!70!black] (5.1440,21) circle (0.55pt);
\node[anchor=east] at (-43,22) {Bubble sort};
\draw[blue!70!black,line width=.45pt] (-4.6592,22)--(18.2920,22);
\draw[blue!70!black] (-4.6592,21.84)--(-4.6592,22.16);
\draw[blue!70!black] (18.2920,21.84)--(18.2920,22.16);
\fill[blue!70!black] (6.8164,22) circle (0.55pt);
\node[anchor=east] at (-43,23) {Dijkstra};
\draw[blue!70!black,line width=.45pt] (-0.9851,23)--(15.6531,23);
\draw[blue!70!black] (-0.9851,22.84)--(-0.9851,23.16);
\draw[blue!70!black] (15.6531,22.84)--(15.6531,23.16);
\fill[blue!70!black] (7.3340,23) circle (0.55pt);
\node[anchor=east] at (-43,24) {Graham scan};
\draw[blue!70!black,line width=.45pt] (7.0738,24)--(28.6945,24);
\draw[blue!70!black] (7.0738,23.84)--(7.0738,24.16);
\draw[blue!70!black] (28.6945,23.84)--(28.6945,24.16);
\fill[blue!70!black] (17.8842,24) circle (0.55pt);
\node[anchor=east] at (-43,25) {Quicksort};
\draw[blue!70!black,line width=.45pt] (3.1321,25)--(39.1140,25);
\draw[blue!70!black] (3.1321,24.84)--(3.1321,25.16);
\draw[blue!70!black] (39.1140,24.84)--(39.1140,25.16);
\fill[blue!70!black] (21.1230,25) circle (0.55pt);
\node[anchor=east] at (-43,26) {Prim};
\draw[blue!70!black,line width=.45pt] (6.7566,26)--(36.3782,26);
\draw[blue!70!black] (6.7566,25.84)--(6.7566,26.16);
\draw[blue!70!black] (36.3782,25.84)--(36.3782,26.16);
\fill[blue!70!black] (21.5674,26) circle (0.55pt);
\node[anchor=east] at (-43,27) {Insertion sort};
\draw[blue!70!black,line width=.45pt] (30.2250,27)--(56.8942,27);
\draw[blue!70!black] (30.2250,26.84)--(30.2250,27.16);
\draw[blue!70!black] (56.8942,26.84)--(56.8942,27.16);
\fill[blue!70!black] (43.5596,27) circle (0.55pt);
\node[anchor=east] at (-43,28) {Binary search};
\draw[blue!70!black,line width=.45pt] (33.9253,28)--(58.1255,28);
\draw[blue!70!black] (33.9253,27.84)--(33.9253,28.16);
\draw[blue!70!black] (58.1255,27.84)--(58.1255,28.16);
\fill[blue!70!black] (46.0254,28) circle (0.55pt);
\node[anchor=east,text=gray] at (-43,29) {optimal\_bst};
\node[anchor=west,text=gray] at (-2,29) {shared failure};
\node at (12,-2.35) {Difference in official CLRS score (percentage points)};
\end{tikzpicture}


==> img/tikz/routing_operator.tex <==
eb\begin{tikzpicture}[
  font=\scriptsize,
  head/.style={circle,draw,minimum size=4.5mm,inner sep=0pt},
  route/.style={-{Latex[length=1.6mm]},thick},
  faded/.style={route,gray!55},
  cross/.style={route,blue!70!black}
]
\node[font=\bfseries,align=center] at (-2.2,1.35) {Attention\quad\(D\) diagonal};
\foreach \y/\lab in {0.75/1,0/2,-0.75/3}{
  \node[head] (ls\lab) at (-3.2,\y) {\lab};
  \node[head] (lr\lab) at (-1.2,\y) {\lab};
  \draw[faded] (ls\lab) -- node[above,sloped,font=\tiny] {\(\alpha^{(\lab)}\)} (lr\lab);
}
\node[font=\tiny,align=center] at (-2.2,-1.25) {heads are stalk coordinates;\\only \(h\!\to\!h\) messages};
\draw[gray!40] (0,-1.4)--(0,1.4);
\node[font=\bfseries,align=center] at (2.35,1.35) {OffDiag\quad\(D+O\)};
\foreach \y/\lab in {0.75/1,0/2,-0.75/3}{
  \node[head] (rs\lab) at (1.25,\y) {\lab};
  \node[head] (rr\lab) at (3.45,\y) {\lab};
}
\draw[faded] (rs1)--node[above,sloped,font=\tiny]{\(\alpha^{(1)}\)}(rr1);
\draw[faded] (rs2)--node[above,sloped,font=\tiny]{\(\alpha^{(2)}\)}(rr2);
\draw[faded] (rs3)--node[above,sloped,font=\tiny]{\(\alpha^{(3)}\)}(rr3);
\draw[cross] (rs1)--node[above,sloped,font=\tiny]{\(O^{21}\)}(rr2);
\draw[cross] (rs3)--node[below,sloped,font=\tiny]{\(O^{13}\)}(rr1);
\draw[cross] (rs2)--(rr3);
\node[font=\tiny,align=center] at (2.35,-1.25) {edge-specific \(s\!\to\!r\) routes\\before neighbor summation};
\end{tikzpicture}


==> tables/clrs_all_tasks.tex <==
\begin{longtable}{lrrrrr}
\caption{Full CLRS results over ten paired seeds. Model scores are mean \(\pm\) seed SD in percent; the difference column is mean paired difference \(\pm\) paired-seed SD in percentage points, followed by its paired 95\% \(t\)-interval. The final column counts seeds with higher/equal/lower OffDiag score.}\label{tab:clrs-all}\\
\toprule Task & GATv2 (\%) & OffDiag (\%) & Difference \(\pm\) SD (pp) & 95\% CI (pp) & \(+/0/-\) \\
\midrule\endfirsthead
\toprule Task & GATv2 (\%) & OffDiag (\%) & Difference \(\pm\) SD (pp) & 95\% CI (pp) & \(+/0/-\) \\
\midrule\endhead
Binary search & 28.32\(\pm\)13.36 & 74.35\(\pm\)11.36 & +46.03\(\pm\)16.91 & [+33.93,+58.13] & 10/0/0 \\
Insertion sort & 9.55\(\pm\)9.16 & 53.11\(\pm\)17.69 & +43.56\(\pm\)18.64 & [+30.22,+56.89] & 10/0/0 \\
Prim & 37.22\(\pm\)19.62 & 58.79\(\pm\)11.08 & +21.57\(\pm\)20.70 & [+6.76,+36.38] & 8/0/2 \\
Quicksort & 10.73\(\pm\)9.22 & 31.85\(\pm\)25.87 & +21.12\(\pm\)25.15 & [+3.13,+39.11] & 7/0/3 \\
Graham scan & 57.86\(\pm\)10.13 & 75.74\(\pm\)10.90 & +17.88\(\pm\)15.11 & [+7.07,+28.69] & 8/0/2 \\
Dijkstra & 77.19\(\pm\)7.93 & 84.52\(\pm\)7.09 & +7.33\(\pm\)11.63 & [-0.99,+15.65] & 8/0/2 \\
Bubble sort & 7.62\(\pm\)8.36 & 14.44\(\pm\)15.16 & +6.82\(\pm\)16.04 & [-4.66,+18.29] & 6/0/4 \\
Matrix chain & 75.87\(\pm\)4.16 & 81.01\(\pm\)4.54 & +5.14\(\pm\)5.99 & [+0.86,+9.43] & 8/0/2 \\
Topological sort & 74.47\(\pm\)12.37 & 78.44\(\pm\)16.98 & +3.97\(\pm\)19.03 & [-9.64,+17.58] & 8/0/2 \\
DFS & 20.22\(\pm\)5.66 & 23.57\(\pm\)6.10 & +3.35\(\pm\)8.52 & [-2.74,+9.44] & 6/0/4 \\
Floyd--Warshall & 18.82\(\pm\)9.34 & 21.59\(\pm\)5.60 & +2.77\(\pm\)12.43 & [-6.11,+11.66] & 5/0/5 \\
Bellman--Ford & 88.15\(\pm\)1.87 & 90.89\(\pm\)1.76 & +2.74\(\pm\)1.67 & [+1.55,+3.94] & 10/0/0 \\
DAG shortest paths & 94.98\(\pm\)3.55 & 97.36\(\pm\)1.80 & +2.38\(\pm\)2.42 & [+0.65,+4.12] & 9/0/1 \\
Minimum & 87.76\(\pm\)7.93 & 90.07\(\pm\)3.80 & +2.31\(\pm\)6.21 & [-2.13,+6.75] & 7/0/3 \\
Kadane & 61.38\(\pm\)2.18 & 62.42\(\pm\)3.34 & +1.04\(\pm\)3.11 & [-1.18,+3.27] & 6/0/4 \\
Bridges & 33.16\(\pm\)7.37 & 34.06\(\pm\)5.15 & +0.90\(\pm\)8.10 & [-4.89,+6.70] & 4/0/6 \\
LCS length & 84.29\(\pm\)0.78 & 84.55\(\pm\)1.18 & +0.26\(\pm\)1.06 & [-0.50,+1.03] & 7/0/3 \\
KMP & 0.01\(\pm\)0.02 & 0.27\(\pm\)0.40 & +0.26\(\pm\)0.41 & [-0.03,+0.55] & 5/4/1 \\
Naive string & 3.82\(\pm\)1.81 & 3.94\(\pm\)1.38 & +0.12\(\pm\)2.17 & [-1.43,+1.67] & 6/0/4 \\
Jarvis march & 59.78\(\pm\)2.39 & 59.85\(\pm\)2.66 & +0.07\(\pm\)4.18 & [-2.92,+3.06] & 6/0/4 \\
Quickselect & 0.00\(\pm\)0.00 & 0.02\(\pm\)0.06 & +0.02\(\pm\)0.06 & [-0.02,+0.06] & 1/9/0 \\
BFS & 99.98\(\pm\)0.03 & 99.97\(\pm\)0.03 & -0.00\(\pm\)0.03 & [-0.02,+0.01] & 1/7/2 \\
Task scheduling & 82.09\(\pm\)1.60 & 81.67\(\pm\)2.07 & -0.41\(\pm\)3.08 & [-2.62,+1.79] & 5/0/5 \\
Segments intersect & 80.04\(\pm\)0.76 & 79.33\(\pm\)0.97 & -0.71\(\pm\)1.44 & [-1.74,+0.32] & 3/0/7 \\
Articulation points & 36.39\(\pm\)8.28 & 33.37\(\pm\)13.08 & -3.02\(\pm\)17.20 & [-15.33,+9.29] & 5/0/5 \\
Activity selector & 56.80\(\pm\)13.24 & 53.61\(\pm\)3.99 & -3.20\(\pm\)14.19 & [-13.35,+6.96] & 3/0/7 \\
SCC & 33.77\(\pm\)6.85 & 30.44\(\pm\)7.33 & -3.33\(\pm\)9.57 & [-10.18,+3.51] & 4/0/6 \\
Kruskal & 63.12\(\pm\)3.27 & 59.04\(\pm\)6.07 & -4.08\(\pm\)6.76 & [-8.92,+0.76] & 4/0/6 \\
Heapsort & 42.66\(\pm\)28.79 & 37.98\(\pm\)14.98 & -4.68\(\pm\)37.42 & [-31.45,+22.08] & 5/0/5 \\
\bottomrule
\end{longtable}


==> tables/clrs_families.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2.6pt}
\caption{Exploratory CLRS family summary. Scores are task-macro means in percent; the final column counts tasks with a positive mean paired difference.}
\label{tab:clrs-families}
\begin{tabular}{lrrrrr}
\toprule
Family & Tasks & GATv2 (\%) & OffDiag (\%) & Difference (pp) & Positive\\
\midrule
Graph/path/connectivity & 12 & 56.46 & 59.34 & +2.88 & 8/12\\
Sorting & 4 & 17.64 & 34.34 & +16.70 & 3/4\\
Search/selection & 3 & 38.69 & 54.81 & +16.12 & 3/3\\
Geometry & 3 & 65.89 & 71.64 & +5.75 & 2/3\\
DP/sequence & 3 & 73.85 & 76.00 & +2.15 & 3/3\\
String matching & 2 & 1.92 & 2.11 & +0.19 & 2/2\\
Scheduling/greedy & 2 & 69.44 & 67.64 & -1.80 & 0/2\\
\midrule
Overall & 29 & 49.17 & 55.04 & +5.87 & 21/29\\
\bottomrule
\end{tabular}
\end{table}


==> tables/clrs_macros.tex <==
\newcommand{\ClrsBootLo}{+1.58}
\newcommand{\ClrsBootHi}{+10.91}


==> tables/feature_main.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3.0pt}
\caption{Test accuracy (\%, mean \(\pm\) standard deviation over ten fixed splits). \(V\) and \(O\) denote the vanilla and \offdiag{} variants; subscripts \(D\) and \(P\) denote dense and partitioned inputs. Partition effects are partitioned minus dense, and positive \(\featureDelta\) indicates reduced sensitivity for \offdiag{}. Means and partition effects are rounded independently; \(\featureDelta\) is the difference of the displayed partition effects.}
\label{tab:feature-main}
\begin{tabular}{lrrrrrrr}
\toprule
Dataset & \(V_D\) & \(O_D\) & \(V_P\) & \(O_P\) & \(\Delta V\) & \(\Delta O\) & \(\featureDelta\)\\
\midrule
\multicolumn{8}{l}{\textit{GATv2 backbone}}\\
Roman Empire & \(86.8{\pm}0.3\) & \(84.5{\pm}0.7\) & \(77.3{\pm}0.7\) & \(84.3{\pm}0.4\) & \(-9.6\) & \(-0.2\) & \(+9.4\)\\
Amazon Ratings & \(46.1{\pm}0.7\) & \(46.2{\pm}0.7\) & \(44.7{\pm}0.5\) & \(46.3{\pm}0.6\) & \(-1.4\) & \(+0.1\) & \(+1.5\)\\
Squirrel Filtered & \(38.9{\pm}1.3\) & \(39.6{\pm}2.2\) & \(37.7{\pm}1.5\) & \(39.1{\pm}2.0\) & \(-1.2\) & \(-0.5\) & \(+0.7\)\\
Chameleon Filtered & \(39.9{\pm}3.3\) & \(37.6{\pm}3.6\) & \(40.6{\pm}3.2\) & \(41.9{\pm}4.5\) & \(+0.7\) & \(+4.3\) & \(+3.6\)\\
\midrule
\multicolumn{8}{l}{\textit{Graph-Transformer backbone}}\\
Roman Empire & \(87.6{\pm}0.4\) & \(86.7{\pm}0.5\) & \(83.7{\pm}0.5\) & \(85.4{\pm}0.4\) & \(-4.0\) & \(-1.3\) & \(+2.7\)\\
Amazon Ratings & \(43.7{\pm}0.4\) & \(44.7{\pm}1.3\) & \(43.6{\pm}0.5\) & \(45.6{\pm}0.8\) & \(-0.0\) & \(+0.9\) & \(+0.9\)\\
Squirrel Filtered & \(39.8{\pm}2.6\) & \(38.1{\pm}2.2\) & \(38.7{\pm}1.3\) & \(40.0{\pm}2.0\) & \(-1.0\) & \(+1.9\) & \(+2.9\)\\
Chameleon Filtered & \(39.6{\pm}2.4\) & \(38.3{\pm}3.8\) & \(41.3{\pm}2.6\) & \(39.6{\pm}3.5\) & \(+1.7\) & \(+1.3\) & \(-0.4\)\\
\bottomrule
\end{tabular}
\end{table}


==> tables/main_movielens.tex <==
\begin{table}[t]
\centering
\caption{\emph{Link Prediction on MovieLens-100K.} We evaluate over 10 seeds, reporting mean $\pm$ std 
$\times 100$. $\Delta$ is the seed-paired improvement of \model{} over its
baseline.}
\label{tab:heterogeneous}
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{llcccc}
\toprule
Model & Variant & AUROC & AUPR & $\Delta$AUROC & $\Delta$AUPR \\
\midrule
GATv2 & -- 
      & $88.70 \pm 0.83$ 
      & $86.48 \pm 1.07$ 
      & -- 
      & -- \\

GATv2 & Top-A
      & $\mathbf{90.35 \pm 0.44}$ 
      & $\mathbf{88.57 \pm 0.54}$
      & $+1.65$ 
      & $+2.10$ \\
\midrule
GT & -- 
   & $81.26 \pm 3.67$ 
   & $76.24 \pm 5.21$ 
   & -- 
   & -- \\

GT & Top-A
   & $\mathbf{90.20 \pm 0.85}$ 
   & $\mathbf{88.38 \pm 0.99}$
   & $+8.94$ 
   & $+12.14$ \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/proof-of-concept_Main.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.7}
\caption{
Feature-isolation results on \textsc{Roman-Empire} with
\(H=4\), \(C=64\), and \(L=5\). Accuracy is reported as
mean \(\pm\) standard deviation over ten splits.
}
\label{tab:roman-fixed-proof}
\resizebox{0.60\columnwidth}{!}{%
\begin{tabular}{lrrrr}
\toprule
\textbf{Model}
& \textbf{Dense}
& \textbf{Split}
& \(\boldsymbol{\delta}\)
& \(\boldsymbol{\Delta_{\mathrm{route}}}\) \\
\midrule
GATv2
& \(86.1{\pm}0.3\)
& \(67.1{\pm}1.5\)
& \(-19.0\)
& -- \\

\gats{}
& \(84.8{\pm}0.4\)
& \(78.0{\pm}0.8\)
& \(-6.8\)
& \(\mathbf{+12.2}\) \\
\midrule

GT
& \(84.9{\pm}0.4\)
& \(72.9{\pm}0.5\)
& \(-12.0\)
& -- \\

\gts{}
& \(86.2{\pm}0.5\)
& \(85.6{\pm}1.0\)
& \(\mathbf{-0.6}\)
& \(\mathbf{+11.4}\) \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/star_results.tex <==
\begin{table}[h]
\centering
\caption{STaR relation-classification accuracy (\%) averaged equally over $b=1,\ldots,8$, $k=2,\ldots,15$ and three seeds. GATv2 and Graph Transformer (GT) use 15 shared-weight recurrent rounds and train on $b=1,2,3$, $k=2,3,4$. Both variants use edge relations in attention; Top-A additionally activates the off-diagonal controller. Bold indicates the better variant within each architecture.}
\label{tab:star-results}
\small
\resizebox{0.4\linewidth}{!}{%
\begin{tabular}{llrr}
\toprule
Architecture & Variant & RCC-8 & Interval Algebra \\
\midrule
GATv2 & -- & 39.79 & 18.05 \\
 & Top-A & \textbf{51.79} & \textbf{52.44} \\
\midrule
GT & -- & 34.05 & 7.69 \\
 & Top-A & \textbf{57.91} & \textbf{52.10} \\
\bottomrule
\end{tabular}%
}
\end{table}
